Random matrix theory improved Fr\'echet mean of symmetric positive definite matrices

In this study, we consider the realm of covariance matrices in machine learning, particularly focusing on computing Fr\'echet means on the manifold of symmetric positive definite matrices, commonly referred to as Karcher or geometric means. Such means are leveraged in numerous machine-learning tasks. Relying on advanced statistical tools, we introduce a random matrix theory-based method that estimates Fr\'echet means, which is particularly beneficial when dealing with low sample support and a high number of matrices to average. Our experimental evaluation, involving both synthetic and real-world EEG and hyperspectral datasets, shows that we largely outperform state-of-the-art methods.

==> Figures/mse_nmatrices/5_25/output.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
width=\columnwidth,
height=4cm,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Number of matrices},
xmin=2.2437647322819, xmax=1337.03857487278,
xmode=log,
xtick style={color=black},
xtick={0.1,1,10,100,1000,10000,100000},
xticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\)
},
y grid style={darkgray176},
ylabel={MSE},
ymin=0.000379717971279199, ymax=20.1375303129162,
ymode=log,
ytick style={color=black},
ytick={1e-05,0.0001,0.001,0.01,0.1,1,10,100,1000},
yticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\)
}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:3,1.00111691885235)
--(axis cs:3,0.242662351506986)
--(axis cs:5,0.163221302129445)
--(axis cs:20,0.0780933248622451)
--(axis cs:30,0.073562719369156)
--(axis cs:40,0.0715116867740018)
--(axis cs:60,0.0675163750600415)
--(axis cs:80,0.0688651332729055)
--(axis cs:100,0.0689308857032579)
--(axis cs:1000,0.0743048560270507)
--(axis cs:1000,0.105052514567065)
--(axis cs:1000,0.105052514567065)
--(axis cs:100,0.136630628469856)
--(axis cs:80,0.151747410388139)
--(axis cs:60,0.157045002201535)
--(axis cs:40,0.189221097709762)
--(axis cs:30,0.205596166051169)
--(axis cs:20,0.271233850899762)
--(axis cs:5,0.628482264113363)
--(axis cs:3,1.00111691885235)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:3,12.13555385122)
--(axis cs:3,8.93652083178367)
--(axis cs:5,9.25126149157753)
--(axis cs:20,9.66889083367207)
--(axis cs:30,9.79754417185975)
--(axis cs:40,9.85450545926054)
--(axis cs:60,9.92433898298992)
--(axis cs:80,9.94940436153678)
--(axis cs:100,10.0086614354127)
--(axis cs:1000,10.1934231185474)
--(axis cs:1000,10.3745241955988)
--(axis cs:1000,10.3745241955988)
--(axis cs:100,10.5648394017509)
--(axis cs:80,10.5941642503707)
--(axis cs:60,10.6392962811557)
--(axis cs:40,10.7218086423827)
--(axis cs:30,10.8092916653157)
--(axis cs:20,10.9533699187732)
--(axis cs:5,11.6028123200417)
--(axis cs:3,12.13555385122)
--cycle;

\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:3,12.2815776729252)
--(axis cs:3,9.44328359347)
--(axis cs:5,9.79054769703643)
--(axis cs:20,10.1812987877089)
--(axis cs:30,10.2635015903304)
--(axis cs:40,10.3269740172121)
--(axis cs:60,10.3975711261742)
--(axis cs:80,10.43312797331)
--(axis cs:100,10.4650638577213)
--(axis cs:1000,10.6198964124901)
--(axis cs:1000,10.7807681514766)
--(axis cs:1000,10.7807681514766)
--(axis cs:100,10.9531337372961)
--(axis cs:80,10.9732930511024)
--(axis cs:60,11.0264844260148)
--(axis cs:40,11.1207262559774)
--(axis cs:30,11.1683909575603)
--(axis cs:20,11.2761192082818)
--(axis cs:5,11.9139859240684)
--(axis cs:3,12.2815776729252)
--cycle;

\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:3,0.690931467599105)
--(axis cs:3,0.206219207260978)
--(axis cs:5,0.14510210542033)
--(axis cs:20,0.0948519988141808)
--(axis cs:30,0.089681912341369)
--(axis cs:40,0.0918892596422362)
--(axis cs:60,0.092118389580167)
--(axis cs:80,0.0952253421601221)
--(axis cs:100,0.097604956828388)
--(axis cs:1000,0.108470580186441)
--(axis cs:1000,0.139813549239583)
--(axis cs:1000,0.139813549239583)
--(axis cs:100,0.167369321658288)
--(axis cs:80,0.172111214225925)
--(axis cs:60,0.183501078893765)
--(axis cs:40,0.202017108103555)
--(axis cs:30,0.218945976003984)
--(axis cs:20,0.245585349092971)
--(axis cs:5,0.495715555534937)
--(axis cs:3,0.690931467599105)
--cycle;

\path [fill=black, fill opacity=0.2]
(axis cs:3,0.794318934700682)
--(axis cs:3,0.21637240879828)
--(axis cs:5,0.131316283900395)
--(axis cs:20,0.0331722272946312)
--(axis cs:30,0.021649675024175)
--(axis cs:40,0.0162019228464954)
--(axis cs:60,0.0106635138506762)
--(axis cs:80,0.0078405015134601)
--(axis cs:100,0.0063496262976184)
--(axis cs:1000,0.0006226058541201)
--(axis cs:1000,0.0021538830893464)
--(axis cs:1000,0.0021538830893464)
--(axis cs:100,0.0216262414400377)
--(axis cs:80,0.0270677899044086)
--(axis cs:60,0.0373148080352239)
--(axis cs:40,0.0568307965558478)
--(axis cs:30,0.0771502807932365)
--(axis cs:20,0.114242923177177)
--(axis cs:5,0.443383024766154)
--(axis cs:3,0.794318934700682)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
3 0.561803044679663
5 0.372785036853189
20 0.179474625108256
30 0.143976940239739
40 0.144965931008824
60 0.122471664251872
80 0.122251731403312
100 0.113571055810565
1000 0.114853176532061
};
\addlegendentry{SCM}
\addplot [semithick, darkorange25512714]
table {%
3 10.4952751372028
5 10.4100832183256
20 10.3128793582248
30 10.3008149630267
40 10.288634572172
60 10.2887083705405
80 10.2747889284676
100 10.2835187064137
1000 10.281949648189
};
\addlegendentry{LW linear}
\addplot [semithick, forestgreen4416044]
table {%
3 10.89702763455
5 10.8308375664196
20 10.7225329134666
30 10.7137319401956
40 10.7104421615176
60 10.7113947362119
80 10.7038714258237
100 10.7050678575276
1000 10.6998167554028
};
\addlegendentry{OAS}
\addplot [semithick, crimson2143940]
table {%
3 0.431596273303805
5 0.305730000712655
20 0.172086794045216
30 0.152926116067352
40 0.151737695108779
60 0.138622803351817
80 0.137723753115095
100 0.133427856149854
1000 0.124500946921857
};
\addlegendentry{LW nonlinear}
\addplot [semithick, black]
table {%
3 0.460079303501696
5 0.271485128543989
20 0.0682589839891463
30 0.0455971037537456
40 0.0342338614296108
60 0.0223472202386557
80 0.016535800668534
100 0.0133605802455973
1000 0.0013178391989009
};
\addlegendentry{RMT}

\legend{};
\end{axis}

\end{tikzpicture}


==> Figures/mse_nmatrices/5_7/output.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
width=\columnwidth,
height=4cm,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=lightgray204,
},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Number of matrices},
xmin=1.99975742259766, xmax=15001.8195512086,
xmode=log,
xtick style={color=black},
xtick={0.1,1,10,100,1000,10000,100000,1000000},
xticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{6}}\)
},
y grid style={darkgray176},
ylabel={MSE},
ymin=0.00449219404204775, ymax=25.4244437132536,
ymode=log,
ytick style={color=black},
ytick={0.0001,0.001,0.01,0.1,1,10,100,1000},
yticklabels={
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\)
}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:3,7.73187675409498)
--(axis cs:3,1.7827542506651)
--(axis cs:5,1.50861963718579)
--(axis cs:20,1.44931469219117)
--(axis cs:30,1.43765752689627)
--(axis cs:40,1.47154816186774)
--(axis cs:60,1.50483828571556)
--(axis cs:80,1.52446841608792)
--(axis cs:100,1.56616240082775)
--(axis cs:1000,1.28475593080161)
--(axis cs:10000,1.84337809143339)
--(axis cs:10000,1.92901411457523)
--(axis cs:10000,1.92901411457523)
--(axis cs:1000,2.01502326276734)
--(axis cs:100,2.3274299105081)
--(axis cs:80,2.42962880245902)
--(axis cs:60,2.5312614375959)
--(axis cs:40,2.64176462167929)
--(axis cs:30,2.81510282570014)
--(axis cs:20,3.13121679966485)
--(axis cs:5,5.43034722270887)
--(axis cs:3,7.73187675409498)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:3,16.0831737791907)
--(axis cs:3,11.4633150122748)
--(axis cs:5,11.6722420377039)
--(axis cs:20,12.4335699943671)
--(axis cs:30,12.5402393610521)
--(axis cs:40,12.7100113085043)
--(axis cs:60,12.8036645104771)
--(axis cs:80,12.8701523693237)
--(axis cs:100,12.9149940416845)
--(axis cs:1000,13.2073265455226)
--(axis cs:10000,13.3053153922831)
--(axis cs:10000,13.4052173058351)
--(axis cs:10000,13.4052173058351)
--(axis cs:1000,13.5104129732433)
--(axis cs:100,13.7827853397935)
--(axis cs:80,13.8465473596733)
--(axis cs:60,13.9363075504161)
--(axis cs:40,14.0932667523803)
--(axis cs:30,14.1890946829044)
--(axis cs:20,14.352497063013)
--(axis cs:5,15.4952991018758)
--(axis cs:3,16.0831737791907)
--cycle;

\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:3,17.1660337292102)
--(axis cs:3,13.1951287523227)
--(axis cs:5,13.4652510315394)
--(axis cs:20,14.142725865054)
--(axis cs:30,14.2009775010935)
--(axis cs:40,14.3422183072233)
--(axis cs:60,14.4485515751155)
--(axis cs:80,14.507787997236)
--(axis cs:100,14.5332007094121)
--(axis cs:1000,14.7608617532422)
--(axis cs:10000,14.8312145805619)
--(axis cs:10000,14.9095914225919)
--(axis cs:10000,14.9095914225919)
--(axis cs:1000,14.9946634650127)
--(axis cs:100,15.2524101812697)
--(axis cs:80,15.2663532483258)
--(axis cs:60,15.3411915608526)
--(axis cs:40,15.4913630033431)
--(axis cs:30,15.5670908157253)
--(axis cs:20,15.639146164438)
--(axis cs:5,16.5965514429272)
--(axis cs:3,17.1660337292102)
--cycle;

\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:3,3.72015574684649)
--(axis cs:3,0.856626954084607)
--(axis cs:5,0.711538223796842)
--(axis cs:20,0.556845179910406)
--(axis cs:30,0.584144326546762)
--(axis cs:40,0.601566963293289)
--(axis cs:60,0.628832774386386)
--(axis cs:80,0.639490092208931)
--(axis cs:100,0.652544906277396)
--(axis cs:1000,0.768564116239764)
--(axis cs:10000,0.811703390618186)
--(axis cs:10000,0.859437137277634)
--(axis cs:10000,0.859437137277634)
--(axis cs:1000,0.913274736134684)
--(axis cs:100,1.09279243498997)
--(axis cs:80,1.15749153257207)
--(axis cs:60,1.19476446520727)
--(axis cs:40,1.28193639708558)
--(axis cs:30,1.39540722912561)
--(axis cs:20,1.5508874449488)
--(axis cs:5,2.79660080964429)
--(axis cs:3,3.72015574684649)
--cycle;

\path [fill=black, fill opacity=0.2]
(axis cs:3,4.77706581153115)
--(axis cs:3,1.23270773299328)
--(axis cs:5,0.672460348936679)
--(axis cs:20,0.154983530284246)
--(axis cs:30,0.107235728001765)
--(axis cs:40,0.0816794494554721)
--(axis cs:60,0.0539271900294134)
--(axis cs:80,0.0422099879393748)
--(axis cs:100,0.0349574459137343)
--(axis cs:1000,0.0073632302535324)
--(axis cs:10000,0.0066533444109871)
--(axis cs:10000,0.0112002436460964)
--(axis cs:10000,0.0112002436460964)
--(axis cs:1000,0.0226440358902968)
--(axis cs:100,0.126210185470559)
--(axis cs:80,0.1552488377403)
--(axis cs:60,0.196539334522303)
--(axis cs:40,0.277966179652569)
--(axis cs:30,0.391265163367051)
--(axis cs:20,0.553227255878865)
--(axis cs:5,2.54599211944222)
--(axis cs:3,4.77706581153115)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
3 4.21730246502197
5 3.26880330232017
20 2.21985162396872
30 2.11494684003525
40 2.04787442316871
60 2.00501179044876
80 1.97818051411886
100 1.94698832741726
1000 1.86926877799498
10000 1.87142180555832
};
\addlegendentry{SCM}
\addplot [semithick, darkorange25512714]
table {%
3 13.6982041928477
5 13.5455256487854
20 13.3984465887753
30 13.3871673402771
40 13.3928958414766
60 13.3694174077518
80 13.3654657071871
100 13.3541586054222
1000 13.3579583569628
10000 13.3546680104195
};
\addlegendentry{LW linear}
\addplot [semithick, forestgreen4416044]
table {%
3 15.0626845147761
5 15.0044714537239
20 14.8983212086522
30 14.8847728885298
40 14.8967874896113
60 14.8782808534378
80 14.8772017974207
100 14.8754287054181
1000 14.8723143886389
10000 14.8713980754615
};
\addlegendentry{OAS}
\addplot [semithick, crimson2143940]
table {%
3 2.09555534133798
5 1.60692541331856
20 1.02155799209649
30 0.956004931127738
40 0.9183125581994
60 0.893984627887419
80 0.882177909488513
100 0.875282431801983
1000 0.839444609671896
10000 0.835466553760627
};
\addlegendentry{LW nonlinear}
\addplot [semithick, black]
table {%
3 2.60078831124017
5 1.46267098067891
20 0.336548306944534
30 0.227576701283793
40 0.167207045241825
60 0.115519872748896
80 0.0882834243912138
100 0.0707646537215089
1000 0.014468975220009
10000 0.0087388812046504
};
\addlegendentry{RMT}

\legend{};
\end{axis}

\end{tikzpicture}


==> Figures/mse_nmatrices/64_128/output.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
width=\columnwidth,
height=4cm,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Number of matrices},
xmin=2.2437647322819, xmax=1337.03857487278,
xmode=log,
xtick style={color=black},
xtick={0.1,1,10,100,1000,10000,100000},
xticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\)
},
y grid style={darkgray176},
ylabel={MSE},
ymin=0.0218043651445638, ymax=56.0024815737763,
ymode=log,
ytick style={color=black},
ytick={0.001,0.01,0.1,1,10,100,1000},
yticklabels={
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\)
}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:3,18.8043389613054)
--(axis cs:3,16.8314875609603)
--(axis cs:5,12.1381896526981)
--(axis cs:20,7.40333054447914)
--(axis cs:30,6.99241936580442)
--(axis cs:40,6.84333140532385)
--(axis cs:60,6.5547090007593)
--(axis cs:80,6.44242941841111)
--(axis cs:100,6.42923176293192)
--(axis cs:1000,6.15031714334588)
--(axis cs:1000,9.57269828056928)
--(axis cs:1000,9.57269828056928)
--(axis cs:100,9.77214297162595)
--(axis cs:80,6.84651314814767)
--(axis cs:60,7.03283275125054)
--(axis cs:40,10.1446648799031)
--(axis cs:30,7.5899688263652)
--(axis cs:20,8.04034681130094)
--(axis cs:5,13.6925881202131)
--(axis cs:3,18.8043389613054)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:3,39.005998009636)
--(axis cs:3,36.8707156277165)
--(axis cs:5,35.5865352644737)
--(axis cs:20,34.5473070558395)
--(axis cs:30,34.579891613708)
--(axis cs:40,34.5237197996682)
--(axis cs:60,34.5172640777862)
--(axis cs:80,34.5040367785707)
--(axis cs:100,34.5406761244513)
--(axis cs:1000,34.6100474756888)
--(axis cs:1000,34.7667457265176)
--(axis cs:1000,34.7667457265176)
--(axis cs:100,35.018072659898)
--(axis cs:80,35.0204169989352)
--(axis cs:60,35.1346156589806)
--(axis cs:40,35.3105106802022)
--(axis cs:30,35.4543696924228)
--(axis cs:20,35.6181967536497)
--(axis cs:5,37.4501666134047)
--(axis cs:3,39.005998009636)
--cycle;

\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:3,39.1942675122421)
--(axis cs:3,37.2808363913984)
--(axis cs:5,35.7911711661596)
--(axis cs:20,34.8860863353065)
--(axis cs:30,34.8716226124352)
--(axis cs:40,34.7987963431535)
--(axis cs:60,34.7593184055425)
--(axis cs:80,34.7893520398673)
--(axis cs:100,34.7844604342404)
--(axis cs:1000,34.8937987135023)
--(axis cs:1000,35.0518189132013)
--(axis cs:1000,35.0518189132013)
--(axis cs:100,35.2747395820992)
--(axis cs:80,35.280664789503)
--(axis cs:60,35.3843482742359)
--(axis cs:40,35.491153530183)
--(axis cs:30,35.7177289930558)
--(axis cs:20,35.9151745882271)
--(axis cs:5,37.7412903329415)
--(axis cs:3,39.1942675122421)
--cycle;

\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:3,13.4150106353578)
--(axis cs:3,11.6981243465868)
--(axis cs:5,9.61827227403283)
--(axis cs:20,7.36444461877267)
--(axis cs:30,7.14352133961181)
--(axis cs:40,7.00841372147705)
--(axis cs:60,6.94320751913582)
--(axis cs:80,6.91012783163816)
--(axis cs:100,6.74522525628883)
--(axis cs:1000,6.69264725683738)
--(axis cs:1000,6.94221203330159)
--(axis cs:1000,6.94221203330159)
--(axis cs:100,7.30551547212458)
--(axis cs:80,7.36045805216695)
--(axis cs:60,7.29151580346628)
--(axis cs:40,7.60690213210427)
--(axis cs:30,8.48945039975636)
--(axis cs:20,8.00543821354113)
--(axis cs:5,10.6273361853284)
--(axis cs:3,13.4150106353578)
--cycle;

\path [fill=black, fill opacity=0.2]
(axis cs:3,13.2493448302234)
--(axis cs:3,11.4860534270566)
--(axis cs:5,6.42575481512846)
--(axis cs:20,1.47633412090066)
--(axis cs:30,0.984704248724723)
--(axis cs:40,0.745685316007821)
--(axis cs:60,0.495193991616838)
--(axis cs:80,0.37902380712767)
--(axis cs:100,0.304820634372988)
--(axis cs:1000,0.0311550294148225)
--(axis cs:1000,0.0341197901365598)
--(axis cs:1000,0.0341197901365598)
--(axis cs:100,0.335310339716903)
--(axis cs:80,0.418883868889403)
--(axis cs:60,0.564439336906844)
--(axis cs:40,0.825173648165352)
--(axis cs:30,1.09302438447952)
--(axis cs:20,1.6280331731264)
--(axis cs:5,7.12816348512381)
--(axis cs:3,13.2493448302234)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
3 17.8578669661773
5 12.8155686738752
20 7.73639624547268
30 7.34216999141405
40 7.25532560940202
60 6.85056244981613
80 6.72031984059409
100 6.7701088293971
1000 6.60524420674127
};
\addlegendentry{SCM}
\addplot [semithick, darkorange25512714]
table {%
3 37.9287812137695
5 36.510870869585
20 35.1182093437605
30 34.9814035545661
40 34.8926849163795
60 34.8302189752921
80 34.7929360698527
100 34.7916496247899
1000 34.6521177061983
};
\addlegendentry{LW linear}
\addplot [semithick, forestgreen4416044]
table {%
3 38.1727186345762
5 36.786643404877
20 35.3985798037799
30 35.2478541588808
40 35.1524144312998
60 35.0782768971115
80 35.0594873887069
100 35.0314417745551
1000 34.9673991259342
};
\addlegendentry{OAS}
\addplot [semithick, crimson2143940]
table {%
3 12.3112936200546
5 10.0392129332778
20 7.68102260267098
30 7.48727072899839
40 7.50180091565585
60 7.30395299485244
80 7.16727107641064
100 7.12028507303887
1000 6.98447855227814
};
\addlegendentry{LW nonlinear}
\addplot [semithick, black]
table {%
3 12.279626119493
5 6.77618065458479
20 1.55136016011359
30 1.04161989750938
40 0.785323043157254
60 0.528655778789545
80 0.399959956704565
100 0.320227137484716
1000 0.0325302658364751
};
\addlegendentry{RMT}

\legend{};
\end{axis}

\end{tikzpicture}


==> Figures/mse_nmatrices/64_128/plot_legend.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
width=\columnwidth,
height=6cm,
legend cell align={left},
legend columns=4, 
legend style={draw=none, at={(0.01, 0.01)},anchor=south west, /tikz/column 2/.style={column sep=5pt,}},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Number of matrices},
xmin=2.2437647322819, xmax=1337.03857487278,
xmode=log,
xtick style={color=black},
minor xtick={2,3,4,5,6,7,8,9,20,30,40,50,60,70,80,90,200,300,400,500,600,700,800,900,2000,3000,4000,5000,6000,7000,8000,9000},
xtick={0.1,1,10,100,1000,10000,100000},
xticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\)
},
y grid style={darkgray176},
ylabel={MSE},
ymin=0.0218043651445638, ymax=56.0024815737763,
ymode=log,
ytick style={color=black},
ytick={0.001,0.01,0.1,1,10,100,1000},
yticklabels={
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\)
}
]
\path [fill=red, fill opacity=0.2]
(axis cs:3,18.8043389613054)
--(axis cs:3,16.8314875609603)
--(axis cs:5,12.1381896526981)
--(axis cs:20,7.40333054447914)
--(axis cs:30,6.99241936580442)
--(axis cs:40,6.84333140532385)
--(axis cs:60,6.5547090007593)
--(axis cs:80,6.44242941841111)
--(axis cs:100,6.42923176293192)
--(axis cs:1000,6.15031714334588)
--(axis cs:1000,9.57269828056928)
--(axis cs:1000,9.57269828056928)
--(axis cs:100,9.77214297162595)
--(axis cs:80,6.84651314814767)
--(axis cs:60,7.03283275125054)
--(axis cs:40,10.1446648799031)
--(axis cs:30,7.5899688263652)
--(axis cs:20,8.04034681130094)
--(axis cs:5,13.6925881202131)
--(axis cs:3,18.8043389613054)
--cycle;

\path [fill=blue, fill opacity=0.2]
(axis cs:3,39.005998009636)
--(axis cs:3,36.8707156277165)
--(axis cs:5,35.5865352644737)
--(axis cs:20,34.5473070558395)
--(axis cs:30,34.579891613708)
--(axis cs:40,34.5237197996682)
--(axis cs:60,34.5172640777862)
--(axis cs:80,34.5040367785707)
--(axis cs:100,34.5406761244513)
--(axis cs:1000,34.6100474756888)
--(axis cs:1000,34.7667457265176)
--(axis cs:1000,34.7667457265176)
--(axis cs:100,35.018072659898)
--(axis cs:80,35.0204169989352)
--(axis cs:60,35.1346156589806)
--(axis cs:40,35.3105106802022)
--(axis cs:30,35.4543696924228)
--(axis cs:20,35.6181967536497)
--(axis cs:5,37.4501666134047)
--(axis cs:3,39.005998009636)
--cycle;

% \path [fill=forestgreen4416044, fill opacity=0.2]
% (axis cs:3,39.1942675122421)
% --(axis cs:3,37.2808363913984)
% --(axis cs:5,35.7911711661596)
% --(axis cs:20,34.8860863353065)
% --(axis cs:30,34.8716226124352)
% --(axis cs:40,34.7987963431535)
% --(axis cs:60,34.7593184055425)
% --(axis cs:80,34.7893520398673)
% --(axis cs:100,34.7844604342404)
% --(axis cs:1000,34.8937987135023)
% --(axis cs:1000,35.0518189132013)
% --(axis cs:1000,35.0518189132013)
% --(axis cs:100,35.2747395820992)
% --(axis cs:80,35.280664789503)
% --(axis cs:60,35.3843482742359)
% --(axis cs:40,35.491153530183)
% --(axis cs:30,35.7177289930558)
% --(axis cs:20,35.9151745882271)
% --(axis cs:5,37.7412903329415)
% --(axis cs:3,39.1942675122421)
% --cycle;

\path [fill=orange, fill opacity=0.2]
(axis cs:3,13.4150106353578)
--(axis cs:3,11.6981243465868)
--(axis cs:5,9.61827227403283)
--(axis cs:20,7.36444461877267)
--(axis cs:30,7.14352133961181)
--(axis cs:40,7.00841372147705)
--(axis cs:60,6.94320751913582)
--(axis cs:80,6.91012783163816)
--(axis cs:100,6.74522525628883)
--(axis cs:1000,6.69264725683738)
--(axis cs:1000,6.94221203330159)
--(axis cs:1000,6.94221203330159)
--(axis cs:100,7.30551547212458)
--(axis cs:80,7.36045805216695)
--(axis cs:60,7.29151580346628)
--(axis cs:40,7.60690213210427)
--(axis cs:30,8.48945039975636)
--(axis cs:20,8.00543821354113)
--(axis cs:5,10.6273361853284)
--(axis cs:3,13.4150106353578)
--cycle;

\path [fill=black, fill opacity=0.2]
(axis cs:3,13.2493448302234)
--(axis cs:3,11.4860534270566)
--(axis cs:5,6.42575481512846)
--(axis cs:20,1.47633412090066)
--(axis cs:30,0.984704248724723)
--(axis cs:40,0.745685316007821)
--(axis cs:60,0.495193991616838)
--(axis cs:80,0.37902380712767)
--(axis cs:100,0.304820634372988)
--(axis cs:1000,0.0311550294148225)
--(axis cs:1000,0.0341197901365598)
--(axis cs:1000,0.0341197901365598)
--(axis cs:100,0.335310339716903)
--(axis cs:80,0.418883868889403)
--(axis cs:60,0.564439336906844)
--(axis cs:40,0.825173648165352)
--(axis cs:30,1.09302438447952)
--(axis cs:20,1.6280331731264)
--(axis cs:5,7.12816348512381)
--(axis cs:3,13.2493448302234)
--cycle;

\addplot [semithick, red]
table {%
3 17.8578669661773
5 12.8155686738752
20 7.73639624547268
30 7.34216999141405
40 7.25532560940202
60 6.85056244981613
80 6.72031984059409
100 6.7701088293971
1000 6.60524420674127
};
\addlegendentry{SCM}
\addplot [semithick, blue]
table {%
3 37.9287812137695
5 36.510870869585
20 35.1182093437605
30 34.9814035545661
40 34.8926849163795
60 34.8302189752921
80 34.7929360698527
100 34.7916496247899
1000 34.6521177061983
};
\addlegendentry{LW}
% \addplot [semithick, forestgreen4416044]
% table {%
% 3 38.1727186345762
% 5 36.786643404877
% 20 35.3985798037799
% 30 35.2478541588808
% 40 35.1524144312998
% 60 35.0782768971115
% 80 35.0594873887069
% 100 35.0314417745551
% 1000 34.9673991259342
% };
% \addlegendentry{OAS}
\addplot [semithick, orange]
table {%
3 12.3112936200546
5 10.0392129332778
20 7.68102260267098
30 7.48727072899839
40 7.50180091565585
60 7.30395299485244
80 7.16727107641064
100 7.12028507303887
1000 6.98447855227814
};
\addlegendentry{LW-NL}
\addplot [semithick, black]
table {%
3 12.279626119493
5 6.77618065458479
20 1.55136016011359
30 1.04161989750938
40 0.785323043157254
60 0.528655778789545
80 0.399959956704565
100 0.320227137484716
1000 0.0325302658364751
};
\addlegendentry{RMT}

\end{axis}

\end{tikzpicture}


==> Figures/mse_nmatrices/64_512/output.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
width=\columnwidth,
height=4cm,
legend cell align={left},
legend style={
  fill=none,
  draw=none,
  text opacity=1,
  at={(1.7,0.5)},
  anchor=east,
},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Number of matrices},
xmin=2.2437647322819, xmax=1337.03857487278,
xmode=log,
xtick style={color=black},
xtick={0.1,1,10,100,1000,10000,100000},
xticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\)
},
y grid style={darkgray176},
ylabel={MSE},
ymin=0.00415627686359689, ymax=22.9910398888739,
ymode=log,
ytick style={color=black},
ytick={0.0001,0.001,0.01,0.1,1,10,100,1000},
yticklabels={
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\)
}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:3,4.34568073915104)
--(axis cs:3,2.49715444557313)
--(axis cs:5,1.5541725764222)
--(axis cs:20,0.569750336387955)
--(axis cs:30,0.471527340456061)
--(axis cs:40,0.425279481700036)
--(axis cs:60,0.370695473539714)
--(axis cs:80,0.34773402837591)
--(axis cs:100,0.333344644130872)
--(axis cs:1000,0.283635904763365)
--(axis cs:1000,0.390070123464593)
--(axis cs:1000,0.390070123464593)
--(axis cs:100,1.12515888326207)
--(axis cs:80,0.924980216884235)
--(axis cs:60,0.976886822139371)
--(axis cs:40,1.12433719088557)
--(axis cs:30,0.838008854609256)
--(axis cs:20,0.864287206754695)
--(axis cs:5,1.81527720271553)
--(axis cs:3,4.34568073915104)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:3,15.4572551307876)
--(axis cs:3,14.5532030503795)
--(axis cs:5,13.6277463055423)
--(axis cs:20,12.73572512538)
--(axis cs:30,12.650143383762)
--(axis cs:40,12.6063917784642)
--(axis cs:60,12.5554652751274)
--(axis cs:80,12.5458602059471)
--(axis cs:100,12.5399866983485)
--(axis cs:1000,12.5372493393955)
--(axis cs:1000,12.5955429536977)
--(axis cs:1000,12.5955429536977)
--(axis cs:100,12.7083425971744)
--(axis cs:80,12.7166821401443)
--(axis cs:60,12.777377831737)
--(axis cs:40,12.8657342192473)
--(axis cs:30,12.9311048464825)
--(axis cs:20,13.0927631034037)
--(axis cs:5,14.3112574459357)
--(axis cs:3,15.4572551307876)
--cycle;

\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:3,15.5392080387105)
--(axis cs:3,14.5921332907271)
--(axis cs:5,13.6605294381209)
--(axis cs:20,12.7620085219135)
--(axis cs:30,12.6686283147272)
--(axis cs:40,12.625140164577)
--(axis cs:60,12.5801727939016)
--(axis cs:80,12.5731431571351)
--(axis cs:100,12.5648456539992)
--(axis cs:1000,12.570170301839)
--(axis cs:1000,12.6343032794278)
--(axis cs:1000,12.6343032794278)
--(axis cs:100,12.7401441718932)
--(axis cs:80,12.7419536412524)
--(axis cs:60,12.8021789020656)
--(axis cs:40,12.8912378215572)
--(axis cs:30,12.964754352703)
--(axis cs:20,13.0846259187851)
--(axis cs:5,14.3394656376821)
--(axis cs:3,15.5392080387105)
--cycle;

\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:3,2.62009319380467)
--(axis cs:3,2.31578534724923)
--(axis cs:5,1.53788370345505)
--(axis cs:20,0.720118527041143)
--(axis cs:30,0.627343185927864)
--(axis cs:40,0.595072477516738)
--(axis cs:60,0.550926354549129)
--(axis cs:80,0.529541305456947)
--(axis cs:100,0.515288158539189)
--(axis cs:1000,0.467685135426895)
--(axis cs:1000,0.541558954566687)
--(axis cs:1000,0.541558954566687)
--(axis cs:100,0.870683350326559)
--(axis cs:80,0.908539474829521)
--(axis cs:60,0.600843418411137)
--(axis cs:40,4.50855937059746)
--(axis cs:30,0.714674862291183)
--(axis cs:20,1.08089427515527)
--(axis cs:5,1.95585814762937)
--(axis cs:3,2.62009319380467)
--cycle;

\path [fill=black, fill opacity=0.2]
(axis cs:3,2.5236028514384)
--(axis cs:3,2.23522661481304)
--(axis cs:5,1.30526811174591)
--(axis cs:20,0.308236841441397)
--(axis cs:30,0.20498401944804)
--(axis cs:40,0.154350920135129)
--(axis cs:60,0.102960498309106)
--(axis cs:80,0.0760209169769133)
--(axis cs:100,0.0612922657248862)
--(axis cs:1000,0.0061494206733131)
--(axis cs:1000,0.0068258307369028)
--(axis cs:1000,0.0068258307369028)
--(axis cs:100,0.0673703429723587)
--(axis cs:80,0.0856882995708599)
--(axis cs:60,0.111436841078402)
--(axis cs:40,0.168498988496121)
--(axis cs:30,0.225822453108656)
--(axis cs:20,0.340809507132715)
--(axis cs:5,1.43657054005459)
--(axis cs:3,2.5236028514384)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
3 2.9238564230599
5 1.8072811769545
20 0.919345676207476
30 0.580209667395038
40 0.881275975144439
60 0.643319209203125
80 0.51693219550031
100 0.599676042484522
1000 0.296773814994851
};
\addlegendentry{SCM}
\addplot [semithick, darkorange25512714]
table {%
3 15.0977301189736
5 13.9706675721955
20 12.8926770764052
30 12.7846554629089
40 12.7221574357975
60 12.6588987043624
80 12.639715922664
100 12.6271199492698
1000 12.568008621096
};
\addlegendentry{LW linear}
\addplot [semithick, forestgreen4416044]
table {%
3 15.1800649398778
5 14.0023145960937
20 12.9205304823012
30 12.8155883316733
40 12.7476438084085
60 12.6882578064579
80 12.6649342427405
100 12.6526503055217
1000 12.600939630746
};
\addlegendentry{OAS}
\addplot [semithick, crimson2143940]
table {%
3 2.46364213356185
5 2.02944052688754
20 0.890242640733354
30 0.701432607273057
40 0.864082028347573
60 0.656104922995448
80 0.688450347017866
100 0.670607153482798
1000 0.488372888872541
};
\addlegendentry{LW nonlinear}
\addplot [semithick, black]
table {%
3 2.39217007959268
5 1.36736601360639
20 0.324411722801173
30 0.215447005291765
40 0.161248998452658
60 0.10734829696662
80 0.0802237725112562
100 0.0644007896675308
1000 0.0065073970653709
};
\addlegendentry{RMT}
\end{axis}

\end{tikzpicture}


==> Figures/mse_nmatrices/64_66/output.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
width=\columnwidth,
height=4cm,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=lightgray204
},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Number of matrices},
xmin=2.2437647322819, xmax=1337.03857487278,
xmode=log,
xtick style={color=black},
xtick={0.1,1,10,100,1000,10000,100000},
xticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\)
},
y grid style={darkgray176},
ylabel={MSE},
ymin=0.0676548185109966, ymax=144.054646180187,
ymode=log,
ytick style={color=black},
ytick={0.001,0.01,0.1,1,10,100,1000,10000},
yticklabels={
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\)
}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:3,101.68201754882)
--(axis cs:3,88.1423662873149)
--(axis cs:5,72.3646618018412)
--(axis cs:20,56.3033594985253)
--(axis cs:30,55.2122414783319)
--(axis cs:40,54.4950492410911)
--(axis cs:60,54.3558372086263)
--(axis cs:80,53.9864569962276)
--(axis cs:100,53.7818808983528)
--(axis cs:1000,52.8842317120235)
--(axis cs:1000,54.1727833123211)
--(axis cs:1000,54.1727833123211)
--(axis cs:100,55.8890710915269)
--(axis cs:80,55.6871970646347)
--(axis cs:60,56.5784776906101)
--(axis cs:40,57.5926819637511)
--(axis cs:30,58.5444375596705)
--(axis cs:20,60.5980312773159)
--(axis cs:5,81.2598670477539)
--(axis cs:3,101.68201754882)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:3,50.9399401272127)
--(axis cs:3,47.616536256823)
--(axis cs:5,47.1612726433819)
--(axis cs:20,46.971955455793)
--(axis cs:30,47.0758081405333)
--(axis cs:40,47.0743333453457)
--(axis cs:60,46.9317172587414)
--(axis cs:80,47.0430248464519)
--(axis cs:100,47.0799238425103)
--(axis cs:1000,47.2703348549419)
--(axis cs:1000,47.4727762654529)
--(axis cs:1000,47.4727762654529)
--(axis cs:100,47.7556083668789)
--(axis cs:80,47.8016846942594)
--(axis cs:60,47.8594004527294)
--(axis cs:40,47.9763694452678)
--(axis cs:30,48.0504043908302)
--(axis cs:20,48.4899285925643)
--(axis cs:5,49.631305562104)
--(axis cs:3,50.9399401272127)
--cycle;

\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:3,51.5543217681294)
--(axis cs:3,48.2174174363328)
--(axis cs:5,47.9435416290828)
--(axis cs:20,47.6022899376881)
--(axis cs:30,47.6905471249209)
--(axis cs:40,47.7473683750189)
--(axis cs:60,47.6137157519845)
--(axis cs:80,47.7378059813306)
--(axis cs:100,47.7700646928333)
--(axis cs:1000,47.947629843197)
--(axis cs:1000,48.1690500555604)
--(axis cs:1000,48.1690500555604)
--(axis cs:100,48.4186590813945)
--(axis cs:80,48.4745541082452)
--(axis cs:60,48.5534576983601)
--(axis cs:40,48.6446214322934)
--(axis cs:30,48.8034004170963)
--(axis cs:20,49.0483158707114)
--(axis cs:5,50.2587948881218)
--(axis cs:3,51.5543217681294)
--cycle;

\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:3,31.0620901659341)
--(axis cs:3,25.7814354065144)
--(axis cs:5,22.4151766483135)
--(axis cs:20,18.5613287460143)
--(axis cs:30,18.2068668295756)
--(axis cs:40,18.0053951577646)
--(axis cs:60,18.0719911571276)
--(axis cs:80,18.0540496547627)
--(axis cs:100,17.8175733279627)
--(axis cs:1000,17.9286725829367)
--(axis cs:1000,18.2797926395433)
--(axis cs:1000,18.2797926395433)
--(axis cs:100,18.8026404764028)
--(axis cs:80,18.9858881503917)
--(axis cs:60,19.1340577061154)
--(axis cs:40,19.5820574055868)
--(axis cs:30,19.8302337288776)
--(axis cs:20,20.3582799108111)
--(axis cs:5,26.0822272030139)
--(axis cs:3,31.0620901659341)
--cycle;

\path [fill=black, fill opacity=0.2]
(axis cs:3,43.0134914235546)
--(axis cs:3,37.0492981565219)
--(axis cs:5,19.756909188043)
--(axis cs:20,4.31132775896778)
--(axis cs:30,2.86976889713881)
--(axis cs:40,2.09763141896607)
--(axis cs:60,1.39543284162807)
--(axis cs:80,1.04403044418553)
--(axis cs:100,0.842579436435285)
--(axis cs:1000,0.0958477337284056)
--(axis cs:1000,0.108031285268237)
--(axis cs:1000,0.108031285268237)
--(axis cs:100,0.944582470496131)
--(axis cs:80,1.17145085610537)
--(axis cs:60,1.5782483886311)
--(axis cs:40,2.3540862718306)
--(axis cs:30,3.154578637464)
--(axis cs:20,4.84674945358772)
--(axis cs:5,22.7658116599057)
--(axis cs:3,43.0134914235546)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
3 94.5157592925942
5 75.6586882309294
20 58.353278559489
30 56.8241460264265
40 56.0826200766897
60 55.3597906632788
80 54.9424181564402
100 54.8161336747953
1000 53.7897210817627
};
\addlegendentry{SCM}
\addplot [semithick, darkorange25512714]
table {%
3 49.3613074737249
5 48.483748351865
20 47.6761402802835
30 47.5720824300155
40 47.5095728646513
60 47.4147988906565
80 47.4285959048943
100 47.4332061562883
1000 47.3704802116759
};
\addlegendentry{LW linear}
\addplot [semithick, forestgreen4416044]
table {%
3 49.9280772828501
5 49.1190938760236
20 48.3424993688959
30 48.2593143364372
40 48.1882416288635
60 48.097836189495
80 48.0973273595286
100 48.1184165931483
1000 48.0624897968217
};
\addlegendentry{OAS}
\addplot [semithick, crimson2143940]
table {%
3 28.4039460003532
5 27.3315303143067
20 19.5467182255244
30 19.0379044881684
40 18.8116447240747
60 18.5874615737571
80 18.4667134698607
100 18.3262967067618
1000 18.0866390671002
};
\addlegendentry{LW nonlinear}
\addplot [semithick, black]
table {%
3 39.6510294255462
5 21.2484674975276
20 4.58847604525462
30 3.01179037254277
40 2.22860231661461
60 1.48283062300453
80 1.1099362145875
100 0.892233532399277
1000 0.102898126015732
};
\addlegendentry{RMT}

\legend{};
\end{axis}

\end{tikzpicture}


==> Figures/mse_nsamples/plot.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{orange}{RGB}{255,165,0}

\begin{axis}[
width=\columnwidth,
height=6cm,
legend cell align={left},
legend columns=4, 
legend style={draw=none, at={(0.01, 0.01)},anchor=south west, /tikz/column 2/.style={column sep=5pt,}},
log basis x={10},
log basis y={10},
minor xtick={2,3,4,5,6,7,8,9,20,30,40,50,60,70,80,90,200,300,400,500,600,700,800,900,2000,3000,4000,5000,6000,7000,8000,9000,20000,30000,40000,50000,60000,70000,80000,90000},
% minor xticklabels={
%   \(\displaystyle {2\times10^{0}}\),
%   \(\displaystyle {3\times10^{0}}\),
%   \(\displaystyle {4\times10^{0}}\),
%   ,
%   \(\displaystyle {6\times10^{0}}\),
%   ,
%   ,
%   ,
%   \(\displaystyle {2\times10^{1}}\),
%   \(\displaystyle {3\times10^{1}}\),
%   \(\displaystyle {4\times10^{1}}\),
%   ,
%   \(\displaystyle {6\times10^{1}}\),
%   ,
%   ,
%   ,
%   \(\displaystyle {2\times10^{2}}\),
%   \(\displaystyle {3\times10^{2}}\),
%   \(\displaystyle {4\times10^{2}}\),
%   ,
%   \(\displaystyle {6\times10^{2}}\),
%   ,
%   ,
%   ,
%   \(\displaystyle {2\times10^{3}}\),
%   \(\displaystyle {3\times10^{3}}\),
%   \(\displaystyle {4\times10^{3}}\),
%   ,
%   \(\displaystyle {6\times10^{3}}\),
%   ,
%   ,
%   ,
%   \(\displaystyle {2\times10^{4}}\),
%   \(\displaystyle {3\times10^{4}}\),
%   \(\displaystyle {4\times10^{4}}\),
%   ,
%   \(\displaystyle {6\times10^{4}}\),
%   ,
%   , 
% },
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Number of samples},
xmin=60.2147602812603, xmax=323.840864082435,
xmode=log,
xtick style={color=black},
xtick={1,10,100,200, 300, 1000,10000},
xticklabels={
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {2\times 10^{2}}\),
  \(\displaystyle {3\times 10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\)
},
y grid style={darkgray176},
ylabel={MSE},
ymin=0.906831409439445, ymax=90.2554928922256,
ymode=log,
ytick style={color=black},
ytick={0.01,0.1,1,10,100,1000},
yticklabels={
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\)
}
]
\path [draw=red, fill=red, opacity=0.2]
(axis cs:65,73.2247445919917)
--(axis cs:65,67.0210988231823)
--(axis cs:68,52.12423914182)
--(axis cs:80,28.6114353039675)
--(axis cs:100,15.5891153792994)
--(axis cs:150,6.40828356957247)
--(axis cs:200,3.78637568572336)
--(axis cs:300,1.91857721931963)
--(axis cs:300,2.15837805380407)
--(axis cs:300,2.15837805380407)
--(axis cs:200,4.18032445704443)
--(axis cs:150,7.24587672600992)
--(axis cs:100,17.1466602445678)
--(axis cs:80,31.2747617984987)
--(axis cs:68,56.1631093720537)
--(axis cs:65,73.2247445919917)
--cycle;

\path [draw=blue, fill=blue, opacity=0.2]
(axis cs:65,49.0806460233759)
--(axis cs:65,47.1903059317982)
--(axis cs:68,46.4200578173441)
--(axis cs:80,43.4389546769218)
--(axis cs:100,39.5206046050163)
--(axis cs:150,31.9088267569193)
--(axis cs:200,26.8715562661357)
--(axis cs:300,20.2320580397824)
--(axis cs:300,20.8559627872577)
--(axis cs:300,20.8559627872577)
--(axis cs:200,27.7427289271786)
--(axis cs:150,33.1027747032573)
--(axis cs:100,41.0441492359144)
--(axis cs:80,45.3967295022002)
--(axis cs:68,48.3403090648444)
--(axis cs:65,49.0806460233759)
--cycle;

% \path [draw=green, fill=green, opacity=0.2]
% (axis cs:65,49.7777653993083)
% --(axis cs:65,47.8319788992543)
% --(axis cs:68,47.0386874624597)
% --(axis cs:80,43.9527265017527)
% --(axis cs:100,39.8520883909034)
% --(axis cs:150,32.1237519162816)
% --(axis cs:200,26.9943061075939)
% --(axis cs:300,20.2479584364334)
% --(axis cs:300,20.9179148262478)
% --(axis cs:300,20.9179148262478)
% --(axis cs:200,27.862191264418)
% --(axis cs:150,33.2909703469184)
% --(axis cs:100,41.3596772927665)
% --(axis cs:80,45.8730398492085)
% --(axis cs:68,49.0560000706235)
% --(axis cs:65,49.7777653993083)
% --cycle;

\path [draw=orange, fill=orange, opacity=0.2]
(axis cs:65,61.1628743156342)
--(axis cs:65,19.2140348546755)
--(axis cs:68,20.8485434640044)
--(axis cs:80,18.2332980925187)
--(axis cs:100,12.2929507734754)
--(axis cs:150,6.16176498341179)
--(axis cs:200,3.94970299030961)
--(axis cs:300,2.0989954884747)
--(axis cs:300,2.37088765165282)
--(axis cs:300,2.37088765165282)
--(axis cs:200,4.37233588203709)
--(axis cs:150,6.75169677869756)
--(axis cs:100,13.5634480543811)
--(axis cs:80,20.1356998917069)
--(axis cs:68,23.7826701552846)
--(axis cs:65,61.1628743156342)
--cycle;

\path [draw=black, fill=black, opacity=0.2]
(axis cs:65,10.5617112562306)
--(axis cs:65,9.12069655941015)
--(axis cs:68,8.548743714098)
--(axis cs:80,6.2352226578141)
--(axis cs:100,4.23591137582339)
--(axis cs:150,2.49755917576852)
--(axis cs:200,1.73886813387942)
--(axis cs:300,1.11774395779948)
--(axis cs:300,1.22238663789645)
--(axis cs:300,1.22238663789645)
--(axis cs:200,1.95026144353997)
--(axis cs:150,2.7553833244157)
--(axis cs:100,4.7841646610119)
--(axis cs:80,6.95555567484867)
--(axis cs:68,9.57450414581776)
--(axis cs:65,10.5617112562306)
--cycle;

\addplot [semithick, red]
table {%
65 69.9529340628551
68 54.1397532375746
80 29.8530930237613
100 16.2956815268801
150 6.8234209954466
200 4.00497232460151
300 2.03565650636212
};
\addlegendentry{SCM}
\addplot [semithick, blue]
table {%
65 48.1840354841978
68 47.3937130640074
80 44.4483851116391
100 40.2515744492378
150 32.5450607196298
200 27.3113782520648
300 20.6588302352151
};
\addlegendentry{LW}

\addplot [semithick, orange]
table {%
65 27.1160428106938
68 22.2422927755893
80 19.0747978732908
100 12.9294913223982
150 6.51354772616796
200 4.43829553724617
300 2.2821129477175
};
\addlegendentry{LW-NL}
\addplot [semithick, black]
table {%
65 9.84778024235454
68 9.08087941977742
80 6.5410435708147
100 4.50235050827252
150 2.61314881691979
200 1.84888784799632
300 1.16814092568788
};
\addlegendentry{RMT}
\end{axis}

\end{tikzpicture}


==> full_numerical_results.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{||c||c|c|c|c||}
    \hline
    \multicolumn{5}{|c|}{PhysionetMI, $p=64$, $K=5$, 23 trials/classes, 109 subjects} \\
    \hline
    Paradigm & SCM & LW-SCM & Non Linear LW & RMT-KM \\
    \hline
    [1,3], 80Hz & {\bf 0.493} & 0.397 & $\times$ & 0.49 \\
    \hline
    \hline
    \multicolumn{5}{|c|}{BNCI2014001, $p=22$, $K=4$, 144 trials/classes, 10 subjects} \\
    \hline
    Paradigm & SCM & LW-SCM & Non Linear LW & RMT-KM \\
    \hline
    [0,4], 125Hz & {\bf 0.629} & 0.578 & $\times$ & 0.625 \\
    \hline
    \hline
    \multicolumn{5}{|c|}{Schirrmeister2017, $p=128$, $K=4$, 120 trials/classes, 14 subjects} \\
    \hline
    Paradigm     & SCM         & LW-SCM & Non Linear LW & RMT-KM \\
    \hline
    [0,5], 100Hz & 0.597       & 0.483 & 0.561          & {\bf 0.603} \\
    \hline
    [3,5], 100Hz & {\bf 0.519} & 0.411 & $\times$       & 0.513 \\
    \hline
    \hline
    \multicolumn{5}{|c|}{Cho2017, $p=64$, $K=2$, 100 trials/classes, 53 subjects} \\
    \hline
    Paradigm & SCM & LW-SCM & Non Linear LW & RMT-KM \\
    \hline
    [1,3], 128Hz & 0.615 & 0.609 & 0.601 & {\bf 0.622} \\
    \hline
    [0,3], 128Hz & {\bf 0.623}& 0.611 & $\times$ & 0.618 \\
    \hline
    \hline
    \multicolumn{5}{|c|}{Lee2019, $p=62$, $K=2$, 100 trials/classes, 55 subjects} \\
    \hline
    Paradigm & SCM & LW-SCM & Non Linear LW & RMT-KM \\
    \hline
    [2,3], 100Hz & {\bf 0.666} & 0.642 & 0.626 & 0.66 \\
    \hline
    \hline
    \multicolumn{5}{|c|}{Weibo2014, $p=60$, $K=7$, 80 trials/classes, 10 subjects} \\
    \hline
    Paradigm & SCM & LW-SCM & Non Linear LW & RMT-KM \\
    \hline
    [0,4], 100Hz & {\bf 0.349} & 0.323 & $\times$ & 0.341 \\
    \hline
    [1,3], 100Hz & {\bf 0.409} & 0.349 & $\times$ & 0.403 \\
    \hline
    \hline
    \multicolumn{5}{|c|}{Ofner2017, $p=61$, $K=7$, 60 trials/classes, 15 subjects} \\
    \hline
    Paradigm & SCM & LW-SCM & Non Linear LW & RMT-KM \\
    \hline
    [0,3], 128Hz & 0.176 & 0.166 & $\times$ & 0.185 \\
    \hline
    [1,2], 128Hz & {\bf 0.187} & 0.186 & $\times$ & 0.185 \\
    \hline
    \hline
    \multicolumn{5}{|c|}{MunichMI, $p=128$, $K=2$, 150 trials/classes, 10 subjects} \\
    \hline
    Paradigm & SCM & LW-SCM & Non Linear LW & RMT-KM \\
    \hline
    [0,7], 100Hz & 0.632 & 0.624 & $\times$ & {\bf 0.638} \\
    \hline
    [2,5], 100Hz & {\bf 0.639} & 0.624 & $\times$ & 0.635 \\
    \hline
    \end{tabular}
    \caption{Classification for motor imaging data}
    \label{tab:my_label}
\end{table*}

\begin{table*}
\centering
\begin{tabular}{|c | c || c | c||c | c||c | c||} 
\hline
 \multicolumn{8}{|c|}{Indian Pines} \\

\multicolumn{2}{|c|}{Parameters} & \multicolumn{2}{|c||}{SCM} & \multicolumn{2}{|c||}{LW-SCM} & \multicolumn{2}{|c|}{RMT-KM} \\ [0.5ex] 
\hline
Data size $p$ & Number of samples $n$ & Accuracy & mIou & Accuracy & mIou & Accuracy & mIou \\ [0.5ex] 
\hline\hline
5 & 5 $\times$ 5 & 0.385 & 0.278 & 0.302 & 0.204 & {\bf 0.454} & {\bf 0.367} \\ 
10 & 5 $\times$ 5 & 0.363 & 0.243 & 0.313 & 0.218 & {\bf 0.422} & {\bf 0.301} \\ 
12 & 7 $\times$ 7 & 0.341 & 0.215 & 0.344 & 0.245 & {\bf 0.446} & {\bf 0.320} \\ 
16 & 5 $\times$ 5 & 0.357 & 0.229 & 0.316 & 0.215 & {\bf 0.413} & {\bf 0.284} \\ 
\hline
\multicolumn{8}{|c|}{Salinas} \\
\hline
\multicolumn{2}{|c|}{Parameters} & \multicolumn{2}{|c||}{SCM} & \multicolumn{2}{|c||}{LW-SCM} & \multicolumn{2}{|c|}{RMT-KM} \\ [0.5ex] 
\hline
Data size $p$ & Number of samples $n$ & Accuracy & mIou & Accuracy & mIou & Accuracy & mIou \\ [0.5ex] 
\hline\hline
5 & 5 $\times$ 5 & 0.542 & 0.382 & 0.402 & 0.252 & {\bf 0.777} & {\bf 0.631} \\ 
10 & 7 $\times$ 7 & 0.525 & 0.34 & 0.449 & 0.303 & {\bf 0.746} & {\bf 0.532} \\ 
10 & 9 $\times$ 9 & 0.489 & 0.323 & 0.433 & 0.271 & {\bf 0.603} & {\bf 0.446} \\ 
16 & 11 $\times$ 11 & 0.497 & 0.317 & 0.404 & 0.244 & {\bf 0.632} & {\bf 0.461}\\
\hline 
\multicolumn{8}{|c|}{Pavia University} \\
\hline
\multicolumn{2}{|c|}{Parameters} & \multicolumn{2}{|c||}{SCM} & \multicolumn{2}{|c||}{LW-SCM} & \multicolumn{2}{|c|}{RMT-KM} \\ [0.5ex] 
\hline
Data size $p$ & Number of samples $n$ & Accuracy & mIou & Accuracy & mIou & Accuracy & mIou \\ [0.5ex] 
\hline
5 & 5 $\times$ 5 & {\bf 0.452} & 0.288 & 0.38 & 0.273 & 0.435 & {\bf 0.463} \\ 
10 & 5 $\times$ 5 & 0.44 & 0.291 & - & - & {\bf 0.51} & {\bf 0.451} \\ 
\hline
\multicolumn{8}{|c|}{Pavia} \\
\hline
\multicolumn{2}{|c|}{Parameters} & \multicolumn{2}{|c||}{SCM} & \multicolumn{2}{|c||}{LW-SCM} & \multicolumn{2}{|c|}{RMT-KM} \\ [0.5ex] 
\hline
Data size $p$ & Number of samples $n$ & Accuracy & mIou & Accuracy & mIou & Accuracy & mIou \\ [0.5ex] 
\hline\hline
5 & 5 $\times$ 5 & 0.629 & 0.378 & 0.615 & 0.319 & {\bf 0.819} & {\bf 0.549} \\ 
\hline
\multicolumn{8}{|c|}{KSC} \\
\hline
\multicolumn{2}{|c|}{Parameters} & \multicolumn{2}{|c||}{SCM} & \multicolumn{2}{|c||}{LW-SCM} & \multicolumn{2}{|c|}{RMT-KM} \\ [0.5ex] 
\hline
Data size $p$ & Number of samples $n$ & Accuracy & mIou & Accuracy & mIou & Accuracy & mIou \\ [0.5ex] 
\hline\hline
5 & 5 $\times$ 5 & 0.263 & 0.167 & 0.247 & 0.169 & {\bf 0.377} & {\bf 0.222} \\ 
\hline
\end{tabular}
\caption{Clustering results for hyperspectral images.}
\end{table*}
